Efficient Pretraining Length Scaling

Recent advances in large language models have demonstrated the effectiveness of length scaling during post-training, yet its potential in pre-training remains underexplored. We present the Parallel Hidden Decoding Transformer (\textit{PHD}-Transformer), a novel framework that enables efficient length scaling during pre-training while maintaining inference efficiency. \textit{PHD}-Transformer achieves this through an innovative KV cache management strategy that distinguishes between original tokens and hidden decoding tokens. By retaining only the KV cache of original tokens for long-range dependencies while immediately discarding hidden decoding tokens after use, our approach maintains the same KV cache size as the vanilla transformer while enabling effective length scaling. To further enhance performance, we introduce two optimized variants: \textit{PHD-SWA} employs sliding window attention to preserve local dependencies, while \textit{PHD-CSWA} implements chunk-wise sliding window attention to eliminate linear growth in pre-filling time. Extensive experiments demonstrate consistent improvements across multiple benchmarks.

==> sections/relatedwork.tex <==
\section{Related Work}

%\subsection{Hello World}

\subsection{Latent Thinking Transformers}

% 最开始是pause token系列，然后quiet star类型的
With the success of Chain-of-thought reasoning~\cite{wei2022chain} in the inference stage, researchers have long been interested in developing pretraining language models that can reason itself. In early stage of this topic, ~\citet{goyalthink} propose to insert learnable \textit{pause} tokens randomly in the pretraining sequence, and observes improvement on reasoning benchmarks including GSM8K~\cite{cobbe2021training}, NaturalQ~\cite{kwiatkowski2019natural}, CommonsenseQA~\cite{talmor2018commonsenseqa}, etc. 

With the promising performance and room for improvement, researches diverge into several categories. A line of researches seeks for more dynamic and automatic approaches in inserting these think tokens, which introduces reinforce. Quiet-Star~\citet{zelikman2024quiet} follows this intuition and proposes a reinforce framework to accelerate the training speed . Although most of these works have, the dependency of thinking tokens results in unacceptable inference latency. Moreover, no general experiments are performed on this methods, and the overhead in reinforcement learning in pretraining stages seems unacceptable and unscalable, especially in the era of test-time scaling and reinforcement length scaling.

% cite deepseek R1

Another line of researches seek for recurrent approaches in reusing model parameters. Both ~\citet{chen2025inner,geiping2025scaling} propose to use recurrent transformer block or transformer layer to scale the computation of decoding tokens, either statically or adaptively. However, recurrent models cannot be used in parallel generation, and they often cannot beat the baseline with same model parameters.


\subsection{Redundant KV Cache and KV cache sharing Transformers}
While recurrent models introduce parameter reusing to make a extremely deep model compactable, KV cache sharing also plays an important role in designing efficient transformers, as KV cache occupies large memory size during the inference stage and is time consuming during pre-filling. YOCO~\citet{sun2024you} proposes to use sparse attention to generate the KV cache, and share the KV cache between the first L/2 layers and the last L/2 layers, achieving notable improvement in reducing GPU memory and speedup in the pre-filling stage. KVSharer~\citet{yang2024kvsharer} proposes to share similar KV cache via post-training and also achieves notable lower memory consumption and generation acceleration. ~\citet{wu2024layer}
further extends the KV cache sharing to extreme version, which segments the original transformer into multiple blocks, and share the KV cache across the blocks.

% In another line of research, more and more paper have revealed the redundancy in current KV, and perform extremely. Methods like sparse attention and KV cache compression. 

As a very extreme circumstance, the naive version of \ours with $K=2$, can be viewed as a very extreme version of the combination of KV cache sharing and parameter reusing technique, where a very deep transformer contains 2
blocks of transformer layers that share the same parameters, and share the same KV cache across all blocks. 


\subsection{Sparse Attention}
Previous works have conducted concrete analysis on the redundancy of attention matrix, leading to the spurs of studies on sparse attention on Large Language Models~\cite{ribar2023sparq,zhang2023h2o}. 

From the analysis in MInference~\cite{jiang2024minference}, the attention matrices in existing LLMs are only sparsely activated with specific patterns. ~\citet{jiang2024minference} further distinguishes these patterns into three typical types, including the local window attention pattern, the vertical-slash pattern and the block sparse pattern. Quest~\cite{tang2024quest} proposes data dependent block-wise sparse attention, which adaptively chooses blocks to attend according to the similarity between current token and block anchors. However, the performance of these training-free methods are limited as it suffers from the inconsistency between training and inference. Recently, Native Sparse Attention(NSA)~\cite{yuan2025native} proposes to incorporate block sparse pattern into the training stage, and achieves improvement both in downstream performance and efficiency. In this paper, driven by previous works that local sliding window attention often keeps the most of attention scores of full attention, we only preserve the local window attention for hidden decoding tokens, which helps us achieve significantly reduced KV cache size thus comparable decoding latency with the original transformer.

==> tables/compare_cocomix.tex <==
\begin{table}[tp]
    \centering
    \small
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{c|cc|cccccccc}
    \toprule
    & \makecell{Train Loss.} & \makecell{Eval Loss.} & MMLU & Hella. & ARC-C & ARC-E & PIQA & Wino. & Comm. & Avg. \\
    \midrule
      PHD-Transformer   &   \\
         & \\
    \bottomrule
    \end{tabular}
    \caption{Comparison with hidden COT models}
    \label{tab:compare_diff_baseline}
\end{table}

==> tables/prefill_decode_speed.tex <==
\begin{table}[tp]
    \centering
    \begin{tabular}{c|ccc}
    \toprule
         Model & Pre-fill(s) & Decoding(s/token) & Speed up \\
         \midrule
         \multicolumn{4}{l}{\textit{Prefilling 1k tokens}} \\
         \midrule
         Vanilla Transformer  & 0.036 & & \\
         \ours & & 0.039 & \\
         \ours -3 & & 0.039 & \\
         \oursswa -3 & 0.015 & 0.051 & \\ 
         \ourscswa & & & \\
        \midrule
         \multicolumn{4}{l}{\textit{Prefilling 1k tokens}} \\
         \midrule
         Vanilla Transformer  & & 0.088 & \\
         \ours & & 0.097 & \\
         \ours & & 0.097 & \\
         \oursswa & 0.015 & 0.141 & \\
         \ourscswa & & & \\
         \midrule
         \multicolumn{4}{l}{\textit{Prefilling 1k tokens}} \\
         \midrule
         Vanilla Transformer  & & 0.337 & \\
         \ours & & 0.342 & \\
         \ours -3 & & 0.342 & \\
         \oursswa & 0.015 & 0.513 & \\
         \ourscswa & & & \\
    \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:prefill_decode_speed}
\end{table}

% 这个图明显可以把roofline打出来。也就是明天这里会有一个很好的图

